An Environment for Analyzing Space Optimizations in Call-by-Need Functional Languages

We present an implementation of an interpreter LRPi for the call-by-need calculus LRP, based on a variant of Sestoft's abstract machine Mark 1, extended with an eager garbage collector. It is used as a tool for exact space usage analyses as a support for our investigations into space improvements of call-by-need calculi.

==> eptcsdata.tex <==
\providecommand{\firstpage}{78}
\providecommand{\publicationstatus}{H. Cirstea, S. Escobar (Eds.): Third International Workshop on Rewriting\\ 
Techniques for Program Transformations and Evaluation (WPTE'16).
\\
EPTCS 235, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.235.6}{10.4204/EPTCS.235.6}}
\pdfoutput=1

